TG-Hyperbolicity of Composition of Virtual Knots

The composition of any two nontrivial classical knots is a satellite knot, and thus, by work of Thurston, is not hyperbolic. In this paper, we explore the composition of virtual knots, which are an extension of classical knots that generalize the idea of knots in $S^3$ to knots in $S \times I$ where $S$ is a closed orientable surface. We prove that for any two hyperbolic virtual knots, there is a composition that is hyperbolic. We then obtain strong lower bounds on the volume of the composition using information from the original knots.

==> Changes.tex <==
1. In eliminating surfaces that have boundary on $K$, you need to worry about compressing disks that are (p,q)-curves on the torus from the boundary of the regular neighborhood of $F\cup K$, when that boundary is a torus. I have put in a fix.

2. Rewrote a bunch in parallel intersection curves

3. Rewrote last paragraph of proof of Thm. 3.7.

4. To Do : Are there better resolution figures for Figures 6-9, 11-16, 18, 19?

5. added a few sentences to boundary compatibility paragraph at the end of the introduction. 7/17

6. To do: we define $\#_s$ explicitly for the first time at the end of section 2. However, we use the notation in theorems in the introduction. Need to think about whether this is a problem or not.

7. To do: do we need to include the paragraph about boundaries at the end of section 2? in my mind the answer is no since we have a similar paragraph at the end of section 1. 
9/7: updated the paragraph in introduction, and removed the paragraph at the end of section 2. 

8. A thought/question: the subsection headings are almost identical to the bold headings used to mark sections of the hyperbolicity proofs. Do we need to change the formatting? 

9. Edited first sentence of volume bounds theorems (4.1, 4.2, 4.4) to match the statements in intro. (Using "non-classical" instead of "with genus at least one")

10. TO DO: think about whether we actually want to include the statement of Agol Storm Thurston thm 9.1 in the volume bounds section. If yes, we should probably change the labelling to make it more obvious that it is their theorem and not ours.
